An Algorithm-to-Contract Framework without Demand Queries

Consider costly and time-consuming tasks that add up to the success of a project, and must be fitted into a given time-frame. This is an instance of the classic budgeted maximization (knapsack) problem, which admits an FPTAS. Now assume an agent is performing these tasks on behalf of a principal, who is the one to reap the rewards if the project succeeds. The principal must design a contract to incentivize the agent. Is there still an approximation scheme? In this work we lay the foundations for an algorithm-to-contract framework, which transforms algorithms for combinatorial problems to handle contract design problems subject to the same combinatorial constraints. Our approach diverges from previous works in avoiding the assumption of demand oracle access. As an example, for budgeted maximization, we show how to "lift" the classic FPTAS to the best-possible (approximately-IC) FPTAS for the contract problem. We establish this through our local-to-global framework, in which the local step is to approximately solve a two-sided strengthened variant of the demand problem. The global step then utilizes the local one to find the approximately optimal contract. We apply our framework to a host of combinatorial constraints: multi-dimensional budgets, budgeted matroid, and budgeted matching constraints. In all cases we essentially match the best purely algorithmic approximation. Separately, we also develop a method for multi-agent contract settings. Our method yields the first approximation schemes for multi-agent contract settings that go beyond additive reward functions.

==> conf.tex <==
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algpseudocode}
\RequirePackage[endLComment=]{algpseudocodex}
\usepackage{soul}
\usepackage{lineno}
\usepackage{xcolor}
\usepackage{tablefootnote}
\usepackage{esvect}
\usepackage{bbm}
\usepackage{thmtools}
\usepackage[]{color-edits}
\usepackage[margin=1in]{geometry}
\geometry{letterpaper}
\usepackage{multirow}
\usepackage{nicematrix,tikz}
\usepackage{booktabs}
\usepackage{pifont}
\usepackage{enumitem}
\usepackage{makecell}
\usepackage{url}

% \linenumbers
 
\newcommand{\xmark}{\ding{55}}

\newcommand{\markwithref}[2]{
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}#1\\(\cref{#2})\end{tabular}}
}

\newcommand{\Min}[1]{\raisebox{0.5ex}{\scalebox{0.8}{$\displaystyle \min_{#1}\;$}}}

\newenvironment{proofsketch}{
  \renewcommand{\proofname}{Proof Sketch}\proof}{\endproof}

\definecolor{ForestGreen}{rgb}{0.1333,0.5451,0.1333}
\definecolor{DarkRed}{rgb}{0.65,0,0}
\definecolor{Red}{rgb}{1,0,0}
\let\pdfbookmark\relax
\usepackage[linktocpage=true,backref=page,
pagebackref=false,colorlinks,
linkcolor=DarkRed,citecolor=ForestGreen,urlcolor=ForestGreen]
{hyperref}

\hypersetup{
   hidelinks,
   colorlinks=true,
}

\usepackage[capitalize]{cleveref}

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{example}[theorem]{Example}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{question}[theorem]{Question}

\newcommand{\negA}{\vspace{-0.05in}}
\newcommand{\negB}{\vspace{-0.1in}}
\newcommand{\negC}{\vspace{-0.18in}}
\newcommand{\posA}{\vspace{0.08in}}
\newcommand{\mysection}[1]{\negC\section{#1}\negA}
\newcommand{\mysubsection}[1]{\negB\subsection{#1}\negA}
\newcommand{\mysubsubsection}[1]{\negB\subsubsection{#1}\negA}
\newcommand{\myparagraph}[1]{\par\smallskip\par\noindent{\bf{}#1.~}}

\newcommand{\al}{\alpha}
\newcommand{\se}{\subseteq}
\newcommand{\lm}{\lambda}
\newcommand{\eps}{\varepsilon}
\newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}}
    
\newcommand{\dr}{\mathbb{R}}
\newcommand{\dn}{\mathbb{N}}
\newcommand{\dz}{\mathbb{Z}}

\newcommand{\si}{\mathcal{I}}
\newcommand{\sa}{\mathcal{A}}
\newcommand{\sv}{\mathcal{V}}
\newcommand{\sk}{\mathcal{K}}
\newcommand{\pnp}{\ensuremath{\textsf{P = NP}}}
\newcommand{\pnotnp}{\ensuremath{\textsf{P} \neq \textsf{NP}}}
\newcommand{\drz}{\dr_{\geq 0}}
\newcommand{\alg}{\mathsf{ALG}}

\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}

\newcommand{\sask}{\ensuremath{\textsf{B-SA}}}
\newcommand{\samk}{\ensuremath{\textsf{MB-SA}}}
\newcommand{\mask}{\ensuremath{\textsf{B-MA}}}
\newcommand{\mamk}{\ensuremath{\textsf{MB-MA}}}
\newcommand{\mcp}{\ensuremath{\textsf{Matroid-SA}}}
\newcommand{\bmic}{\ensuremath{\textsf{BMatroid-SA}}}
\newcommand{\match}{\ensuremath{\textsf{BMatch-SA}}}
\newcommand{\OPT}{\mathrm{OPT}}
\newcommand{\ALG}{\mathrm{ALG}}

\addauthor{ITC}{magenta}
\newcommand{\inbal}[1]{{\ITCcomment{#1}}}
\newcommand{\itc}[1]{{\ITCedit{#1}}}
\addauthor{HS}{red}
\newcommand{\hadas}[1]{{\HScomment{#1}}}
\newcommand{\hs}[1]{{\HSedit{#1}}}
\addauthor{GS}{blue}
\newcommand{\gilad}[1]{{\GScomment{#1}}}
\newcommand{\gs}[1]{{\GSedit{#1}}}
\addauthor{IDA}{orange}
\newcommand{\ilan}[1]{{\IDAcomment{#1}}}
\newcommand{\ida}[1]{{\IDAedit{#1}}}

\providecommand{\keywords}[1]
{
  \small	
  \textbf{\textit{Keywords---}} #1
}
